The Dynamics of Gradient Descent for Overparametrized Neural Networks

We consider the dynamics of gradient descent (GD) in overparameterized single hidden layer neural networks with a squared loss function. Recently, it has been shown that, under some conditions, the parameter values obtained using GD achieve zero training error and generalize well if the initial conditions are chosen appropriately. Here, through a Lyapunov analysis, we show that the dynamics of neural network weights under GD converge to a point which is close to the minimum norm solution subject to the condition that there is no training error when using the linear approximation to the neural network. To illustrate the application of this result, we show that the GD converges to a prediction function that generalizes well, thereby providing an alternative proof of the generalization results in Arora et al. (2019).

==> outline.tex <==
Section: Problem Statement:  
- Describe what a neural network is
- Given a dataset and ideally you would like pick theta to minimize the mean-square error (define this) for regression problems 
- Instead of minimizing the mean-square error directly, we use gradient descent (give the algorithm) starting from appropriate initial condition. If you do this, at the end of T iterations, you are going to have some theta^T(S), S:dataset
- The problem is to characterize the generalization error (define this, specify assumptions on the (x,y) distribution for the noisy case, assume the data also came from this distribution...) of theta^T(S)

Subsection: Approach: For the noiseless case (make it clear what it means), this has been done in Du et al. For the noisy case, to the best of our knowledge, the generalization error has not been characterized but Ghorbani et al have obtained a result for the case where one linearizes the neural network w.r.t. theta. Explain what this means.
-Explain the linearization
-For an overparameterized network, there is more than one solution. It is known that GD finds the minimum norm solution. for this problem, using the representer theorem, we get ... as the solution. In the limit as m\rightarrow\infty, we get kernel regression. Montanari's result is stated for kernel regression. This result will apply to our problem in the following manner: decompose the error and argue that if we show that the first term is small, then because the second term is small from Montanari's result, we will get a good bound on generalization. The goal is to show that the first term is small.

Section: The convergence of gradient descent

- ODE part with proofs, some proofs in appendix
- Discrete-time, all proofs in appendix

Subsection: Discussion: 
- noisy case, plug in Montanari's result
- noiseless case (this is an alternative derivation instead of the Rademacher complexity approach in Du et al, derivation in appendix...), see appendix for an alternative proof of the fact that the RKHS can represent any continuous function arbitrarily closely

